An Approximate Generalization of the Okamura-Seymour Theorem

We consider the problem of multicommodity flows in planar graphs. Okamura and Seymour showed that if all the demands are incident on one face, then the cut-condition is sufficient for routing demands. We consider the following generalization of this setting and prove an approximate max flow-min cut theorem: for every demand edge, there exists a face containing both its end points. We show that the cut-condition is sufficient for routing $\Omega(1)$-fraction of all the demands. To prove this, we give a $L_1$-embedding of the planar metric which approximately preserves distance between all pair of points on the same face.

==> junk.tex <==
%Case 1: If $x \in S, y \not\in S$, then any shortest path between $x,y$ uses exactly one edge of $\delta(S)$. Suppose not. Let $Q[x,y]=yy_{1}y_{2} \cdots y_{m}x$ be such a path and $(y_i,y_{i+1}),(y_j,y_{j+1})$ be the first two edges of $\delta(S)$ on the path while traversing from $y$ to $x$. Then, $y_i,y_{j+1}$ lie on $P[u,v]$. Since $Q[x,y]$ is a shortest path between $x,y$, $d_{Q}(y_i,y_{j+1})=d_{G}(y_i,y_{j+1})$. This implies the existence of another shortest path $P[u,x_i] \cup Q[x_i,x_j] \cup Q[x_j,v]$ between $u,v$ that lies strictly inside the closed region defined by the cycle $P_{b}[u,v] \cup P[u,v]$, contradicting property (4) of the claim.\\

%Case 2: $x,y \not \in S$: let $Q[x,y]=y, y_{1}y_{2} \cdots y_{m}x$ be a shortest path between $x,y$ and $(y_i,y_{i+1}),(y_j,y_{j+1})$ be the first two edges of $\delta(S)$ on the path while traversing from $x$ to $y$. Then, $y_i,y_{j+1}$ lie on $P[u,v]$. Since $P[x,y]$ is a shortest path between $x,y$, $d_{Q}(y_i,y_{j+1})=d_{G}(y_i,y_{j+1})$. This implies the existence of another shortest path $P[u,x_i] \cup Q[x_i,x_j] \cup Q[x_j,v]$ between $u,v$ that lies strictly inside the closed region defined by the cycle $P_{b}[u,v] \cup P[u,v]$, contradicting property (4) of the claim.\\

%Case 3: $x,y \in S$: to prove the statement of the lemma, we only need to consider $x,y \in V(b)$. Let $Q[x,y]=x x_{1}x_{2}\cdots x_{m}y$ be a shortest path such that $Q[x,y] \cap \delta(S) \neq \phi$. Since every edge in $\delta(S)$ has one end point on $P[u,v]$, at least 2 vertices of $P[u,v]$ lie on the path $Q[x,y]$. Let $x_i,x_j \in P[u,v]$ such that $u,x_i,x_j,v$ appear on $P[u,v]$ in that order. Observe that $Q[x,x_i] \cup P[x_i,x_j] \cup Q[x_j,y]$ is also a shortest path between $x,y$ and $d_{G}(u,v)+d_{G}(x,y)=d_{G}(u,x_i)+d_{G}(x_i,x_j)+d_{G}(x_j,v)+d_{G}(x,x_i)+d_{G}(x_i,x_j)+d_{G}(x_j,y) \geq d_{G}(u,y)+d_{G}(x,v)=d_{G}(u,x)+d_{G}(x,y)+d_{G}(x,y)+d_{G}(y,v)= d_{G}(x,y)+d_{b}(u,v)$. Hence, $d_{G}(u,v) \geq d_{b}(u,v)$, which contradicts the choice of $(u,v)$ (property (1) in the claim). \end{proof}

%\begin{lemma}
%Let $S$ be a nice cut. Let $\mathcal{S}= \{(S,1)\}$ and $G'$ be obtained by contracting the edges in $\delta(S)$. Then $G'$ is bipartite and $d_{G}(u,v)=d_{G'}(u,v)+\delta_{\mathcal{S}}(u,v)$ for all $u,v \in V(f), f \in B$.
%\end{lemma}
%\begin{proof}
%Every cycle crosses $S$ an even number of times, hence contracting edges of $\delta(S)$ doesn't change the parity of number of edges on it. Since $G$ is bipartite, $G'$ is bipartite as well. Let $P[x,y]$ be the shortest path associated with $S$,$x,y \in V(b), b\in B$. $P_b[x,y]$ is the shortest path on face $b$ between $x,y$.  Proof of the lemma follows from the following claims.
%\begin{claim}
%Let $x_1,y_1 \in P[x,y]$ and $P'[x,y]$ be a path contained inside $C$. Then $d_{P'}(x,y) \geq d_{P}(x,y)+2$.
%\end{claim}
%\begin{proof}
%$d_{P'}(x,y) >  d_{P}(x,y)$, by (4) of Claim \ref{claim: nice cut}. If $d_{P'}(x,y)=d_{P}(x,y)+1$, then $P[x,y] \cup P'[x,y]$ forms an odd cycle, a contradiction. Hence, $d_{P'}(x,y) \geq d_{P}(x,y)+2$.
%\end{proof}
%\begin{claim} \label{claim: shortest path}
%Let $| \{u,v\} \cap S| \neq 1$. Then for any path $Q[u,v]$, $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]| \geq d_{G}(u,v)$.
%\end{claim}
\begin{proof}
Let $u,v \in S$ and let $Q[u,v]$ be a path with minimum value of $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]|$ with least number of edges. If there exists $\alpha,\beta \in Q[u,v] \cap P[x,y]$ such that $Q[\alpha,\beta]$ lies inside $C$, then replacing $Q[\alpha,\beta]$ by $P[\alpha,\beta]$ in $Q[u,v]$ gives a path with smaller number of vertices and same value of $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]|$, a contradiction. Hence, $Q$ contains 0 or 2 edges of $\delta(S)$. If $Q$ doesn't contain any edges of $\delta(S)$, there is nothing to prove. If $Q$ contains 2 edges of $\delta(S)$, then by Lemma \ref{lemma: existence nice cut}, $Q$ can't be a shortest path. Using the fact that $P_{b}[u,v]\cup Q[u,v]$ is an even cycle, statement of the claim follows.\\
If $u,v \not \in S$, we again consider a path $Q[u,v]$ with minimum value of $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]|$ with least number of edges. If there exists $\alpha,\beta \in Q[u,v] \cap P[x,y]$ such that $Q[\alpha,\beta]$ lies inside $C$, then replacing $Q[\alpha,\beta]$ by $P[\alpha,\beta]$ in $Q[u,v]$ gives a path with smaller number of vertices and same value of $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]|$, a contradiction. This means that $Q$ doesn't contain any edges of $S$, which is contrary to our assumption.
\end{proof}
\begin{claim}
Let $| \{u,v\} \cap S| = 1$. Then for any path $Q[u,v]$, $d_{Q}(u,v)-|\delta(S) \cap Q[u,v]| \geq d_{G}(u,v)-1$.
\end{claim}
\begin{proof}
The proof of this claim is similar to Claim \ref{claim: shortest path}.
\end{proof}
\end{proof}

%Let $P[x,y]$ be the shortest path associated with $S$ and $Q[x_1,y_1]$ be a path from $x_1$ to $v$ which uses edges of $\delta(S)$. We show that $d_{Q}(u,v) \geq d_{G}(u,v)+2$, and the statement of the lemma will follow. $Q[u,v]$ uses at least 2 edges of $\delta(S)$, let $(x_{1},y_{1}),(x_{2},y_{2}) \in \delta(S) \cap P[u,v]$ such that $x_{1},y_{2} \in P[x,y]$. Using property (4) of claim \ref{claim: nice cut},  $d_{P}(x_1,y_2) >  d_{Q}(x_{1},y_{2})$. If $d_{Q}(x_{1},y_{2})=d_{P}(x_1,y_2)+1=d_{G}(x_{1},y_{2})$, then $P[x_1,y_2] \cup Q[x_1,y_2]$ is an odd length cycle, a contradiction. Hence, $d_{Q}(x_1,y_2) \geq  d_{P}(x_{1},y_{2})+2=d_{G}(x_1,y_2)+2$


%Suppose $u \in S, v \not \in S$. Lemma \ref{lemma: existence nice cut} states that any shortest $u,v$ path uses at most one edge of $\delta(S)$, hence this is not possible. Suppose $u,v \in S$. Lemma \ref{lemma: existence nice cut} states that any shortest path between $u,v$ doesn't use any edge of $\delta(S)$, hence this is not possible. Suppose $u,v \not \in S$. Let $P[x,y]$ be the shortest path associated with $S$ and $Q[u,v]$ be a path from $u$ to $v$ which uses edges of $\delta(S)$. We show that $d_{Q}(u,v) \geq d_{G}(u,v)+2$, and the statement of the lemma will follow. $Q[u,v]$ uses at least 2 edges of $\delta(S)$, let $(x_{1},y_{1}),(x_{2},y_{2}) \in \delta(S) \cap P[u,v]$ such that $x_{1},y_{2} \in P[x,y]$. Using property (4) of claim \ref{claim: nice cut},  $d_{P}(x_1,y_2) >  d_{Q}(x_{1},y_{2})$. If $d_{Q}(x_{1},y_{2})=d_{P}(x_1,y_2)+1=d_{G}(x_{1},y_{2})$, then $P[x_1,y_2] \cup Q[x_1,y_2]$ is an odd length cycle, a contradiction. Hence, $d_{Q}(x_1,y_2) \geq  d_{P}(x_{1},y_{2})+2=d_{G}(x_1,y_2)+2$ which implies $d_{Q}(u,v) \geq d_{G}(u,v)+2$.


==> legacy.tex <==
%If $R^{\circ}(f_1,u_1,v_1) \cap R^{\circ}(f_2,u_2,v_2) \neq \emptyset$, then there exists an edge $(x_1,y_1) \in S(f_1,u_1,v_1) \setminus S(f_2,u_2,v_2)$ such that $(x_1,y_1)$ is on the unique shortest $(u_1,v_1)$ path $P[u_1,v_1]$ in $R(f_1,u_1,v_1)$ and $x_1,y_1 \in R(f_2,u_2,v_2)$.
        
        %Order the vertices on the path $P[u_1,v_1]$ from $u_1$ to $v_1$ and choose $x, y$ such that (i) $x,y \in S(f_2,u_2,v_2)$ (ii) $x_1,y_1$ come after $x$ but before $y$ in the ordering (iii) no vertex of $S(f_2,u_2,v_2)$ appears between $x$ and $y$ in the ordering. Hence $P[u_1,v_1]=P[u_1,x] \cup P[x,y] \cup P[y,v_1]$ such that (i) $x,y \in S(f_2,u_2,v_2)$ but none of the edges in $P[x,y]$ are on $S(f_2,u_2,v_2)$ (ii) all the vertices in $P[x,y]$ are in $R(f_2,u_2,v_2)$ (iii) $(x_1,y_1)$ is on $P[x,y]$.
    
        %Let $P_1[x,y] \subseteq S(f_2,u_2,v_2)$ be a $x,y$ path such that none of the vertices of $P_1[x,y]$ is on face $f_2$ (such a path exists by Claim \ref{clm:minimality}). Since $R(f_2) \subsetneq R(f_1,u_1,v_1) \cap R(f_2,u_2,v_2)$, it follows by Claim \ref{clm:minimality} that all the edges on $P_1[x,y]$ are a part of the unique shortest $u_2,v_2$ path inside $R(f_2,u_2,v_2)$. We can replace $P_1[x,y]$ by $P[x,y]$ to obtain another shortest $u_2,v_2$ path inside $R(f_2,u_2,v_2)$, which contradicts the minimality of $R(f_2,u_2,v_2)$. 

        %$R(f_1) \subseteq R(f_1,u_1,v_1) \cap R(f_2,u_2,v_2)$ or $R(f_2) \subseteq R(f_1,u_1,v_1) \cap R(f_2,u_2,v_2)$: Without loss of generality, assume that $R(f_1) \subseteq R(f_1,u_1,v_1) \cap R(f_2,u_2,v_2)$. Let $P[u_1,v_1]$ be the unique $u_1,v_1$ shortest path contained inside $R(f_1,u_1,v_1)$. 



        
For the sake of contradiction, assume that there exist $f_1,f_2 \in F_N$ such that $R(S^1_{f_1}) \setminus R(S^1_{f_2}) \neq  \emptyset$ and $R(S^1_{f_2}) \setminus R(S^1_{f_1}) \neq \emptyset$. Then either $R(f_1) \subseteq R(S^1_{f_2})$ or $R(f_1) \cap R(S^1_{f_2}) = \emptyset$. We present the argument for the case when $R(f_1) \subseteq R(S^1_{f_2})$, an analogous argument works for the second case as well. Suppose $R(f_1) \subseteq R(S^1_{f_2})$. Minimality of $R(S^1_{f_1})$ implies that there must exist $u_1,v_1 \in f_1$ such that any shortest path from $u_1$ to $v_1$ exits and enters the region $R(S^1_{f_2})$ at least once. Let $P(u_1,v_1)$ be one such shortest path and $x_1,y_1$ be the first point of entry/last point of exit of $P(u_1,v_1)$ from/into $R(S^1_{f_2})$ respectively. Let $P(x_1,y_1)$ be the portion of the path between $x_1$ and $y_1$ on the cycle $S^1_{f_2}$. Note that $P(x_1,y_1)$ is a path on the boundary of $\overline{R(S^1_{f_2})}$. Since $\overline{R(S^1_{f_2})}$ defines the minimal region containing the support of the metric on $f_2$, there must exist $u_2,v_2 \in f_2$ such that some shortest path between $u_2$ and $v_2$ uses an edge on the path $P(x_1,y_1)$. Let $P(u_2,v_2)$ be such a shortest path and let $x_2,y_2$ be the first and the last point of intersection of $P(u_2,v_2)$ with $P(u_1,v_1)$. Then replacing the portion of the path $P(u_1,v_1)$ between $x_2$ and $y_2$ by portion of the path $P(u_2,v_2)$ between $x_2$ and $y_2$, we obtain a shortest $u_1,v_1$ path contained completely inside $S^1_{f_2}$. This contradicts our choice of $u_1,v_1$. We can use an analogous argument to arrive at a contradiction in case $R(f_1) \subset R(S^1_{f_2})$ and $R(S^1_{f_1}) \subsetneq R(S^1_{f_2})$. 

%Hence such $f_1,f_2$ can't exist and it must be true that $R(S^1_{f_1}) \cap R(S^1_{f_2})= \emptyset$ or $R(S^1_{f_1}) \subseteq R(S^1_{f_2})$ or $R(S^1_{f_2}) \subseteq R(S^1_{f_1})$ for any $f_1,f_2 \in F_N$.

\begin{lemma} \label{lemma:face_support_distinct}
For any $f_1,f_2 \in F_N$, .
\end{lemma}

\begin{proof}
Let $f_1, f_2 \in F_N$ be such that $R=R(S^1_{f_1})=R(S^1_{f_2})$. Let $C$ be the cycle bounding the region $R$ and $(u,v) \in C$. By minimality of $R$, there must exist $u_1,v_1 \in f_1$ and $u_2,v_2 \in f_2$ such that a shortest $u_1-v_1$ and $u_2-v_2$ path uses the edge $(u,v)$ and is contained completely in $R$. Let these shortest $u_1-v_1$ and $u_2-v_2$ path be $P[u_1,v_1]$ and $P[u_2,v_2]$ respectively. Let the region bounded by $f_1$ and $P[u_1,v_1]$ be $R_1$. Let $R_2$ be defined similarly. Using an argument similar to one in Lemma \ref{Lemma: face_support_laminar}, it is easy to see that one can choose $P[u_1,v_1]$ and $P[u_2,v_2]$ such that either $R_1 \subseteq R_2$ or $R_2 \subseteq R_1$. Without loss of generality, let's assume $R_1 \subseteq R_2$. 

Suppose there exists $x,y \in f_1$ such that any shortest path between $x$ and $y$ uses at least one edge not contained inside $R_2 \setminus R(f_2)$. If no such $x,y$ exist then $R(f_1) \subseteq R_2 \setminus R(f_2) \subset R(S^1_{f_2})$, which contradicts our hypothesis. Consider one such $x-y$ shortest path $P[x,y]$. Since $P[x,y]$ uses at least one edge not in $R_2 \setminus R(f_2)$, it crosses the region bounded by $R_2$ and must have vertices in common with $P[u_2,v_2]$. Let $x_1,y_1 \in P[x,y] \cap P[u_2,v_2]$ be the first and last such vertex while traversing from $x$ to $y$. But then, portion of the path $P[x,y]$ between $x_1$ and $y_1$ can be replaced by the portion of the path $P[u_2,v_2]$ between $x_1$ and $y_1$. This implies that there exists a shortest $x,y$ path contained completely inside $R_2 \setminus R(f_2)$. This contradicts our assumption and hence $R=R(S^1_{f_1})=R(S^1_{f_2})$.  
\end{proof}




all the shortest $xy$ paths have to use an edge in $\overline{R(S^1_{f})} \setminus \overline{R(T_{f})}$. By definition, all such $s_1-t_1$ shortest paths are contained completely inside the region $\overline{R(S^1_{f})}$, and hence must enter and exit the region $R(T_f)$ at one of the vertices of $P$. Let $P'$ be one such shortest $s_1-t_1$ path and $x,y \in P$ be the first and last vertex of $P$ in $P'$ (while traversing $P'$ from $x$ to $y$). Since $P$ is itself a shortest path, we can replace the portion of $P'$ between $x$ and $y$ by the portion of $P$ between $x$ and $y$ to obtain another $s_1-t_1$ shortest path which is contained completely inside $\overline{R(T_f)}$. Hence such $s_1-t_1$ can't exist and $\overline{R(T_{f})}$ contains a support of face $f$. This contradicts the minimality of $S^1_f$. Hence, $P\cap I(S^1_f)= \emptyset$ and this completes proof of the lemma.


\begin{lemma} \label{Lemma: face_support_laminar_final}
Let $f_1,f_2 \in F_N$. Then one of the following must hold: $R(S_{f_1}) \cap R(S_{f_2})= \emptyset$ or $R(S_{f_1}) \subset R(S_{f_2})$ or $R(S_{f_2}) \subset R(S_{f_1})$. Furthermore, if $R(f _1) \subset R(S_{f_2})$, then $R(S_{f_1}) \subset R(S_{f_2})$. 
\end{lemma}

%We now describe this property in more detail. By Lemma \ref{Lemma: face_support_laminar}, the set of regions $\{R(S_f)|f\in F_N\}$ form a laminar structure. This implies that there exists a face $f \in F_N$ such that for any $f'\in F_N$, either $R(S_f) \subset R(S_{f'})$ or $R(f) \cap R(S_{f'})=\emptyset$. We call such a face  \textbf{innermost}. Note that there could be multiple innermost faces. 


%(i) $F_N=\emptyset$ (i.e.~the infinite face is possibly the only non-geodesic face) (ii) if $f \in F_N$ is an innermost face, then $S_f$ is $\alpha$-loose and $G \setminus S_f$ is $\alpha$-good. We now show that any length function can be converted into a $\alpha$-good one by modifying the edge lengths by a (multiplicative) factor of at most $\alpha$.


==> old.tex <==
\section{Embedding Geodesic Faces into $L_1$} \label{Geodesic Faces}
In this section, we show an embedding $f$ that achieves a constant distortion for all pair of vertices $u,v$, where $u$ and $v$ lie on the same geodesic face. We make use of Theorem \ref{seymour} to prove this. Theorem \ref{seymour} states that if union of the supply and the demand graph is planar, then the cut condition is sufficient for routing all the demands with congestion 1. It follows from the $\tt{congestion-distortion}$ theorem that given any planar graph $G=(V,E,l)$ and $H=(V,F)$ such that $G+H$ is planar, there exists an embedding $f$ of vertices into $L_1$ such that $||f(u)-f(v)||_{1}=d_{G}(u,v)$ for all $(u,v) \in F$ and $||f(u)-f(v)||_{1} \leq d_{G}(u,v)$ for all $(u,v) \in E$. Furthermore, from the discussion in \ref{Cut-Metric-Embedding Equivalence}, it follows that there exists a weighted collection of cuts $\mathcal{C}$ such that $\delta_{\mathcal{C}}=f$. We may assume that all cuts in $\mathcal{C}$ are central (ie, $G[C]$ and $G[V \setminus C]$ are connected). If not, then there exists a $(C,w_C) \in \mathcal{C}$ such that $G[V \setminus C]$ has connected components $G_{i}=(V_i,E_i,w_i)$ for $i \in [p]$. We modify $\mathcal{C}$ by replacing $(C,w_C)$ by central cuts $(V_1,w_C),(V_2,w_C),\ldots,(V_p,w_C)$. This operation only increases the value of $\delta_{\mathcal{C}}(u,v)$ for any $u,v \in V$. Also, for any edge $(u,v) \in E$, $\delta_{\mathcal{C}}(u,v) \leq d_{G}(u,v)=w_{uv}$, as total weight of cuts separating $(u,v)$ remains same after the operation. Hence, by triangle inequality it follows that $\delta_{\mathcal{C}(u,v)} \leq d_{G}(u,v)$ for all $u,v \in V$. We repeat this operation until no such cuts remain and obtain a cut-metric which consists only of central cuts.

%Hence, there exists a $\mathcal{C}$ such that all cuts in $\mathcal{C}$ are central, $\delta_{\mathcal{C}}=d_{G}(u,v)$ for all $(u,v) \in F$ and $\delta_{\mathcal{C}} \leq d_{G}(u,v)$ for all $(u,v) \in E$.  

Let $A$ be the set of all geodesic faces in $G$. By scaling every edge weight by a factor of 4 and subdividing the edges, we may assume that all the edge weights are 1 and the number of vertices in every cycle is a multiple of 4. We define two demand graphs $H_1=(V,F_1)$ and $H_2=(V,F_2)$ such that $G \cup H_1$ and $G \cup H_2$ are planar. There is exactly one demand edge incident on each face in $H_1$ and $H_2$. Let $F_{i}=  \bigcup_{f \in A} e_{f}^{i}$ for $i=1,2$. Let $u_0,u_2,\ldots,u_{4m-1}$ be the vertices on the cycle associated with the face $f \in A$ in the clockwise order. Then $e_{f}^{1}=(u_0,u_{2m})$ and $e_{f}^{2}=(u_{m},u_{3m})$. Let $\mathcal{C}_i$ be such that $\delta_{\mathcal{C}_i}(u,v)=d_G(u,v)$ for all $(u,v) \in F_i$ and $\delta_{\mathcal{C}_i}(u,v) \leq d_G(u,v)$ for all $(u,v) \in E$ for $i=1,2$. Let $\mathcal{C}=(\mathcal{C}_1+\mathcal{C}_2)/2$. We claim that $\mathcal{C}$ is the desired cut metric. In the following, let $u_{-i}$ denote $u_{4m-i}$ for $i \in [0,4m]$.

\begin{lemma}
Let $F=\{(u,v)| \textit{$\exists f \in A$ such that $u,v \in f$}\}$. Then $\mathcal{C}$ is such that $\delta_{\mathcal{C}}(u,v) \geq d_{G}(u,v)/2$ for all $(u,v) \in F$ and $\delta_{\mathcal{C}}(u,v) \leq d_{G}(u,v)$ for all $(u,v) \in E$.
\end{lemma}

\begin{proof}
Since $\delta_{\mathcal{C}_1}(u,v) \leq d_{G}(u,v)$ and $\delta_{\mathcal{C}_2}(u,v) \leq d_{G}(u,v)$ for all $u,v \in V$, it follows that $\delta_{\mathcal{C}}(u,v) =(\delta_{\mathcal{C}_i}(u,v)+\delta_{\mathcal{C}_i}(u,v) )/2 \leq  d_{G}(u,v)$ for all $u,v \in V$. We now show the other direction. 

Fix a face $f \in A$ and let $V(f)=\{u_0=u_{4m},u_2,\ldots,u_{4m-1}\}$ be the vertices on the cycle associated with $f$ in clockwise order such that $e_{f}^{1}=(u_0,u_{2m}) \in F_1$ and $e_{f}^{2}=(u_{m},u_{3m})\in F_2$. Let $E(f)=\{e_i|e_i=(u_i,u_{i+1}), i \in [0,4m-1]\}$ be the edges of cycle of $f$. From construction, it follows that $\delta_{\mathcal{C}_1}(u_{0},u_{2m})=2m$. Let $\mathcal{C}_{1}^{f}$ be the subset of cuts of $\mathcal{C}_{1}$ which intersect $f$. Let $\mathcal{C}_{1}^{f}=\{(C_i,w_i)\}_{i=1}^{p}$. Then $\delta(C_i) \cap E(f) \neq \phi$ for $i \in [1,p]$. 

Since each $C_i$ corresponds to a circuit in the planar dual of $G$, we have $|\delta(C_i) \cap E(f)| \geq 2$. This implies that each cut separating $u_0,u_{2m}$ intersects at least two of the $e_i$'s. We have
\begin{equation}
4m \geq \sum_{i=0}^{4m-1} d_{G}(e_i) \geq \sum_{i=0}^{4m-1} \delta_{\mathcal{C}_1}(e_i) \geq 2 \sum_{i=1}^{p}w_i \geq  2 \sum_{i:C_i \cap \{u_0,u_{2m}\} \neq \phi}w_{i} \geq 4m. 
\end{equation}
Hence equality holds everywhere and $\delta_{\mathcal{C}_1}(e_i)=d_G(e_i)=1$. It also follows that every cut in $\mathcal{C}_1$ separates $u_0,u_{2m}$ and intersects exactly two of the $e_i'$. 

Recall that for any $u,v \in f$, $\delta_{\mathcal{C}_1}(u,v)$ is equal to the total weight of cuts in $C_1,C_2,\ldots,C_p$ which separate $u,v$. For the purpose of analysis, we define a new set of cuts $\mathcal{X}$ with respect to face $f$ such that $\delta_{\mathcal{X}_1}(u,v) \leq \delta_{\mathcal{C}_{1}^{f}}(u,v)=\delta_{\mathcal{C}_1}(u,v)$ for all $u,v \in f$. Cuts in $\mathcal{X}$ will have a laminar structure which will simplify the calculations immensely. Without loss of generality, we may assume that $u_0 \in C_i,u_{2m} \notin C_i$ for all $i \in [p]$. We say two sets $A,B$ cross if both $A \setminus B$ and $B \setminus A$ are non empty. We construct $\mathcal{X}_1$ in an iterative manner as follows. Initially $\mathcal{X}_1=\{C_1,\ldots,C_p\}$. While there exists a pair of crossing cuts $(A,w_A),(B,w_B)$ in $\mathcal{X}$ with $w_A \geq w_B$, replace them by $(A \cap B,w_B),(A \cup B,w_B)$ and $(A,w_A-w_B)$. The process stops when there are no crossing pair of cuts. 
\begin{claim}
The uncrossing procedure terminates in $O(m^{4})$ iterations.
\end{claim}
\begin{proof}
It is easy to see that the number of crossing pair of cuts decreases by at least 1 after every iteration. Since each cut in $\mathcal{C}_{1}^{f}$ intersects exactly two edges of cycle of $f$, total number of cuts at the start of the procedure is at most $4m^{2}$. This implies that the total number of crossing pairs in the beginning is $O(m^{4})$ and the uncrossing procedure terminates in $O(m^4)$ steps.
\end{proof}
\begin{claim}
All cuts in $\mathcal{X}_1$ separate $u_0,u_{2m}$.
\end{claim}
\begin{proof}
Recall that $u_0 \in C$ and $u_{2m} \notin C$ for all $C \in \mathcal{X}_1$. Hence, $u_0 \in C_i \cap C_j$, $u_{2m} \notin C_i \cap C_j$, $u_0 \in C_i \cup C_j$, $u_{2m} \notin C_i \cup C_j$ for any $i,j \in \mathcal{X}_1$. This shows that after every iteration of uncrossing, all cuts in $\mathcal{X}_1$ continue to separate $u_0,u_{2m}$ and the claim follows. 
\end{proof}
By construction, cuts in $\mathcal{X}_1$ are non-crossing. Also by the discussion above, each cut in $\mathcal{X}_1$ crosses the cycle of $f$ exactly twice and separates $u_0,u_{2m}$. Hence it follows that $\mathcal{X}_1$ consists of cuts of the form $X_{1}^{i}=\{u_{4m-i},u_{4m-i+1},\ldots,u_{4m-1},u_0,u_1,\ldots,u_i\}$ for $i \in [1,2m]$ and weight of every cut is $1$. We construct $\mathcal{X}_2$ with respect to $\mathcal{C}_2$ and $e_{f}^{2}$ similarly. $\mathcal{X}_2$ consists of cuts of form $X_{2}^{i}=\{u_{m-i+1},u_{m-i},\ldots,u_{m},u_{m+1},\ldots,u_{m+i}\}$ for $i \in [1,2m]$ where $u_{-j}=u_{4m-j}$. We need the following claim to finish the proof.
\begin{claim} \label{claim:uncross}
$\delta_{\mathcal{X}_1}(u,v) + \delta_{\mathcal{X}_2}(u,v) \geq d_G(u,v)$ for all $u,v \in f$.
\end{claim}
\begin{proof}
Let $u,v \in V(f)$ for some $f \in A$. Since $f$ is a geodesic face, $d_{G}(u_i,u_j)= \textit{min} \{|i-j|,4m-|i-j|\}$. It follows from structure of $\mathcal{X}_1$ and $\mathcal{X}_2$ that $\delta_{\mathcal{X}_1}(u_i,u_j)=d_{G}(u_i,u_j)$ in the following cases: (1) $i,j \in [0,2m]$ (2) $i,j \in [2m,4m]$ (3) $i,j \in [0,m] \cup [3m,4m-1]$ (4) $i,j \in [m,3m]$. Only remaining cases are : (5) $i\in [0,m],j \in [2m,3m] $ (6) $i \in [m,2m],j \in [3m,4m]$. We do the argument for case (5), other case is similar. By structure of $\mathcal{X}_1$, it follows that $\delta_{\mathcal{X}_1}(u_i,u_j)=4m-i-j$. Similarly, from structure of $\mathcal{X}_2$, it follows that $\delta_{\mathcal{X}_2}(u_i,u_j)=i+j-2m$. Hence, $\delta_{\mathcal{X}_1}(u_i,u_j) + \delta_{\mathcal{X}_2}(u_i,u_j)=2m \geq \textit{min} \{|i-j|,4m-|i-j|\}$ and the lemma follows.
\end{proof}
For any $u,v \in V(f), \delta_{\mathcal{X}_i}(u,v) \leq  \delta_{\mathcal{C}_i}(u,v)$ for $i=1,2$. This follows from the fact that uncrossing a pair of cuts does not increase the total weight of cuts across any pair of vertices. By Claim \ref{claim:uncross}, it follows that $\delta_{\mathcal{C}_1}(u,v)+\delta_{\mathcal{C}_2}(u,v) \geq \delta_{\mathcal{X}_1}(u,v) + \delta_{\mathcal{X}_1}(u,v) \geq 2 d_{G}(u,v)$ for all $u,v \in f$. This finishes the proof of the lemma.
\end{proof}

%Let $A$ be the set of geodesic faces in $G$ and $B$ be the set of faces which are not geodesic. Note that $F(G)=A \cup B$. We show an embedding by finding a set of weighted cuts with low distortion. The procedure runs in two phases. In phase 1, we iteratively find cuts $C$ such that for any $u,v \in f \in B$, any shortest path between $u,v$ uses exactly one edge of $C$ if and only if $u,v$ is separated by $C$. We call such a cut a geodesic cut. We show that if $B$ is non-empty, then we can always find a geodesic cut. We reduce the length of all the edges of $C$ by appropriately chosen $\epsilon$, update the length function and add $(C,\epsilon)$ to our cut set. If some face of $G$ which was previously in $B$ becomes geodesic, we remove it from $B$ and add it to $A$. We repeat the above till $B$ is non-empty. We embed this modified graph so that pair of vertices on a face in $A$ have low distortion. We now describe phase 2. If some face was originally geodesic, embedding in phase 1 gives no guarantee over the distortion for pair of vertices lying on it. If some face is non-geodesic in $G$, in phase 1 we extract cuts until it becomes geodesic. In phase 2, we find an embedding which gives us the residual distance. We again make use of Theorem \ref{seymour} to find such an embedding.  

%For ease of presentation, we also assume that all edges have length 1. This can be done by replacing any edge with length $l>1$ by replacing it with a path of length $l$. Note that this does not change the original shortest path metric in any way.



==> reviews.tex <==
Referee #1 (Remarks to the Author): 

Many definitions and assertions in the paper are incorrect as written. Sometimes authors will be a bit informal in making certain definitions as long as there is an underlying formal definition that one can, possibly with some effort, formulate. It is not the case here, and I need the author to seriously address these current deficiencies. 

My first issues are in Section 4. The major issue is point (5) below. 

(1) A set of edges being the support should be defined for an arbitrary subset of vertices, not just for f which is a face. The definition makes sense in this generality and this might be needed at later points. But perhaps more importantly, this emphasizes that faces are not special with respect to this definition. 

(2) "A support is called minimal if..." Is this notion of minimality used/needed in the rest of the paper? Note that right after defining a minimal support, certain minimal regions are defined where minimality is a different notion. 

(3) I would use the notation R^{\circ}(C) for the (open) interior of the cycle C, and R(C) for the closed interior. One reason is that \overline{...} doesn't typeset very nicely over long expressions like R(S_f^{i+1}), etc. But it's also because in this context overline is often used for set complement. Since the closed region is a bit more natural, I find that R^{\circ}(C) useful in emphasizing that the set is open. 

(4) The notations G \ C and G[C] are bad, as neither one is what the reader would expect, and both conflict with the standard definitions for graphs. 

Later you introduce the set I(C). You should just define I(C) in Section 4 and then use the notation G \ I(C) for removing the vertices contained in the interior. Alternatively, I think it would be fine to overload (and simplify) notation and use G \ R^{\circ}(C) and G[R(C)] for these two subgraphs. 

(5) Most important: Right now, the support of a face f is not well-defined. The paper says "Let S_f^1 be the cycle such that ... is the inclusion-wise minimal region." The author makes no attempt to establish that "the inclusion-wise minimal region" is well-defined. And, indeed, it is not. 

The author says that "Given a fixed planar embedding of G, S_f is a function of edge lengths." I disagree with this assertion as well, for the same reason. 

It is easy to construct examples where there are two possibilities for S_f^1, both of which are inclusion-wise minimal, but such that their intersection is not a support for f. The idea is to consider vertices u,v on some cycle and then add two non-intersecting u-v shortest paths. For a similar reason, S_f is also not well-defined. 


Referee #2 (Remarks to the Author): 

Summary 

The paper proves a constant bound on the flow-cut gap, which is the worst-case ratio between the maximum concurrent flow and sparsest cut, for a class of multicommodity network flow instances. Namely, the bound is shown for instances where the supply graph is planar and for every demand edge, both ends of the edge lie on the same face (but different demand edges may lie on different faces). Okamura and Seymour previously proved that if the supply graph is planar and there is a single face holding the ends of all demand edges, the flow-cut gap is equal to one, of which this result can be seen as an (approximate) generalization. Previous works have considered other planar settings, such as k-outerplanar graphs or in which the demands are incident on only k faces, but those bounds depend on the parameter k. This paper gives a truly constant bound on a natural class of planar instances not covered by previous works. Consequently, it appears to mark a significant step towards the important GNRS conjecture, which asserts that the flow-cut gap for all planar instances is constant. 

To prove this result the following technique is used. It is demonstrated that for any edge-length function, there is an embedding of the graph metric into L_1 with constant distortion. That is, the embedding (1) does not increase the distance of supply edge pairs and (2) only decreases the distances between demand-edge pairs by a constant factor. This is equivalent to bounding the flow-cut gap by the congestion-distortion theorem. Though at a high level this approach has been used previously for flow-cut gap results, many novel techniques are developed to construct an appropriate embedding for this paper's setting. 

A key aspect of the proof are the concepts of geodesic faces and supports. The support of a face is (roughly) the smallest subgraph such that the distances in the subgraph between any two nodes on the face are the same as in the full graph (i.e. only the subgraph is needed to find shortest paths for that face). If a face supports itself, it is called geodesic. The author shows there is a laminar structure to the supports of the non-geodesic faces. 

The embedding is constructed inductively. The length function is reduced slightly to a ``good' length function that satisfies some nice properties on the non-geodesic faces. If every face is geodesic, it is proved that there is a low-distortion embedding. If there is a geodesic face, an appropriate one is selected using the laminar structure and length function properties. The interior of the support is removed, and an embedding is found inductively for the remaining graph. This embedding is converted to an equivalent cut-metric form, which is then extended (with effort) to the whole graph. Each of these steps on its own takes considerable proof, and often has several supporting lemmas in its own section. 

The author ends by noting that while their result does not imply any bounds on integral or half-integral flow-cut gaps, they speculate that their laminar structure and techniques could be used to prove such bounds, or to extend the inductive arguments used for series-parallel or k-outerplanar graphs to more general planar settings. 


Overall Evaluation 

This is a strong and well-written paper. The setting (routing in planar supply graphs where each demand lies on a single face) is an interesting and natural generalization of that of the Okamura-Seymour theorem. The achieved constant bound is impressive, and makes significant strides towards the GNRS conjecture, which is an important open question in multicommodity flows. While on its face the technique of using an L_1 embedding is not novel, the details required to make such an argument work for this setting are novel and technical. The structural results on planar graphs that are proven are also interesting in their own right and possibly applicable elsewhere. 

I cannot see any differences between the SICOMP version of this paper and the FOCS version of the paper. However, the paper feels complete, with a strong result and essentially no missing details. I found the paper generally very readable. Its well-presented outline together with its clear and concise explanations and notation make the paper very approachable despite the level of technical detail in the proofs. In addition to some typos, I have several minor comments about some definitions and theorems (and one of the proofs in particular, namely Lemma 4) that I would like to see addressed, but I did not find any major problems. As such, I recommend a minor revision. 


Detailed Comments for Author 


Page 4, Section 2.2: ``Let... c, d, l be the capacity, demand, and length functions...'. The use of ``the' suggests these are fixed, but for the definition of I these should be quantified over. 

Page 5, section 2.3: ``We refer to delta_C as ... a cut-metric C'. Does ``cut-metric' refer to C or delta_C? 

Page 6, both Section 3 and 4: The intuition for the limit definition of S_f appears to be that S_f needs to both support the face f and *itself*. In that case, isn't the informal definition of G_f, S_f in Section 3 misleading? While it is alluded to that there is more to the definition, and being vague is reasonable at this point, slightly more information might make an initial reading of the true definition of S_f less confusing. 

Page 6, Section 4: 
- Redefining the standard notation G \ C and G[C] is a little confusing, especially since \ and [] are used with their traditional meaning elsewhere in the paper. Moreover, it seems unnecessary, since the "new" G \ C is just G \ I(C), and G[C] could be replaced using a "closed" version of I(C). 
- For the definition of S^1_f, it is not immediately obvious that there is a *unique* inclusion-wise minimal region containing a support of f, or how to compute it (though, I suspect answering the uniqueness question would make the computation clear). 

Page 7, Lemma 2 proof: 
- ``first point of entry/last point of exit... from/into' -> ``into/from' 
- ``Let P(x_1, y_1) be the portion of the path between x_1 and y_1 on the cycle S^1_{f_2}' reads slightly ambiguously. Does ``the path" refer to the path P(u_1, v_1) from the previous sentence (so P(x_1, y_1) is a subpath of P(u_1, v_1))? If so, considering that P(u_1, v_1) enters the open region R(S^1_{f_2}) at x_1 and exits at y_1, I do not see why this subpath from x_1 to y_1 should be on the boundary cycle S^1_{f_2}. 

Page 8, Lemma 4 and its proof: 
- Is this lemma correct as stated? In particular, the proof seems to be assuming that u, v \in S^1_f (i.e. they are on the boundary of S^1_f, and not just on the face f). If u, v \in I(S^1_f) (i.e. in the interior), I am not sure that T_f is well-defined, and it seems as if you can create an example where a shortest u, v path uses other nodes of f that are in the interior of S^1_f. 
- Additionally, in the opposite case where u, v \in S^1_f (i.e. not in the interior), then it seems incorrect to say {u, v} = P \cap I(S^1_f) as in the lemma statement. 
- ``u_1' is used for two different nodes, a node on the path P and then later u_1, v_1 \in f are introduced. 
- I(S_f) in the first paragraph of the proof should be I(S^1_f). 

Page 12, Theorem 10: By "absolute" is it meant that c is also independent of Delta? May be helpful to clarify. 

Page 12, Theorem 11: It should be noted that beta is an absolute constant (i.e. not depending on G). 

Page 14+15, Lemma 6 and its proof: 
- In the statement of the lemma, it does not seem necessary to say that C_i is a contiguous set of vertices, since that is inherent to the definition of ``cut-metric wrt face f' 
- It may be helpful to explicitly note that the half-integral version of Theorem 1 is being used 
- I do not feel the claim ``each central cut corresponds to a (v_i, v_j) path' is obvious. More detail would be appreciated. 
- Is it not possible that, for an edge e = uv, d_G(u, v) may be strictly less than l(e)? In which case it does not suffice to show that the total weight of cuts separating e is less than l(e)? This seems easy to fix however by redefining the capacity to be d_G(u, v). 
- Very minor nit: the proof sometimes conflates the graphs where f^D is a single node and where f^D has been split. For example: ``Each flow path in G^D... (recall that a circuit...)'. In one graph the flows are paths, in the other they are circuits, but the sentence jumps between the two graphs implicitly. 

Page 15, Theorem 12: 
- Is S a supporting cycle for some face? It seems alpha-loose was only defined for supporting cycles. 
- "Let... alpha >= 12 beta be a constant" but alpha was defined previously in the theorem (since S is alpha-loose) 

Page 17, Theorem 13 and its proof: 
- This theorem defines a new constant "c", but Theorem 10 defined an absolute constant named "c". This would not really be worthy of a complaint, except for the fact that the constant "beta" is carried over multiple theorems, so it feels inconsistent. 
- ``z_1: V -> L_1' V should be V_1 

High-level question: the paper makes it straightforward to track the size of the constant bound back to a function of the number given by Theorem 10. Is it possible to get a concrete number for this, or is this a limitation of the Klein, Plotkin, Rao paper? Now, I don't believe this paper *needs* a concrete number, but it would be nice as I can see there being an interest in optimizing the bound, especially if this result is used as a subroutine to prove the GNRS conjecture in the future. 

I also noticed several minor typos: 
- Page 1, 2nd paragraph: "The demand graph, H is" -> "The demand graph H is" 
- Page 1, 2nd paragraph: 6,3 -> 3,6 
- Page 2, Figure 1 caption: "Figure on the right" -> "The Figure on the right" 
- Page 3, before Theorem 1: "classic results identifies" -> "classic result identifies" 
- Page 3 Theorems 1 & 2: Should "eulerian" be capitalized? 
- Page 3, before Lemma 1: "is a part of cycle" -> "is a part of a cycle" 
- Multiple occurrences (Page 3, Page 4, Page 5 Theorems 3, 4, & 6, Page 12 Theorem 11): "length" should be "lengths" or "length function". Also inconsistent whether written "edge length" or "edge-length" 
- Page 5, section 2.3: "we us them" -> "we use them" 
- Page 6, before section 4: "vertices,i.e." missing space 
- Page 7, first paragraph: R(S^f) has f as superscript, should be subscript 
- Page 7, claim 1: "Face" -> "The face" 
- Page 17, conclusions: "both end points of every demand edge is incident" -> "are incident" 


Referee #3 (Remarks to the Author): 

The main result of this paper is an approximate generalization of the Okamura-Seymour theorem in planar graphs, and more specifically, an embedding into L1 preserving terminal distances up to an O(1) factor in the distortion when the endpoints of each terminal pair are on the same face. Note, however, that the number of faces could depend on n, the number of vertices. This is a major progress toward establishing the L1 embedding conjecture. Previous significant results are for a single face (the Okamura-Seymour theorem) or a constant number of faces. 

The technique is also very interesting. There are two types of faces: geodesic faces and non-geodesic faces. Intuitively, if a terminal pair belongs to a geodesic face, then the shortest path in the graph is along the face. A previous work by the same author handles geodesic faces. The real challenge is the non-geodesic faces. The author introduces the notion of the support of a non-geodesic face and proves a very interesting structural result for the supports: they form a laminar family. Another technical ingredient is the notion of an alpha-loose cycle: a cycle is alpha-loose if the shortest path of any two points in the cycle that does not use any vertex of the cycle other than the endpoints is longer than the true shortest path by at least an alpha factor. The author shows that there is always possible to slightly distort the weight function on the edges so that every support cycle of a non-geodesic face is alpha-loose. This is crucially used in an inductive argument: taking a minimal subgraph enclosed by an alpha-loose cycle, embedding (into L1) the inside (using a clever combination of several known tools) and the outside (by recursion) separately, and then gluing the embedding along the cycle. 

The major complaint I have about this paper is its sloppy writing. I had a very difficult time reading the first 10 pages, especially the structural result section. While the overall proof strategy is sound to me, there are some details that I need clarification on; I left more detailed comments below. The proofs of several theorems and lemmas are very topological in nature but have no accompanying figures to illustrate the ideas, which makes them doubly harder to read. I had to draw a lot of figures myself. I think the author should really make an effort to include more supporting figures. 


Overall, the result is significant, and the techniques of this paper are highly non-trivial and clearly pass the bar for SICOMP. But the writing should be going through more rounds of revision. For now, I recommend a major revision. 

========= 

First, I think the author should number each line of your manuscript; it is painful to describe where the errors are. 

P2. Figure 1: It's hard to see the blue/red in the printed paper. Maybe using thin/bold/dotted instead. 

P2. "A cut $S\subseteq V$ is a partition of the vertex set (S,V\setminus S)." This sentence is hard to parse: is it S a cut, or the partition (S,V\setminus S) is a cut? 

P3. Lemma 1: what does it mean for a central set satisfying a cut condition? Do you mean the induced subgraphs of G and H on the set A? Up to this point, the cut condition is defined for a pair of supply and demand graphs, not for a set. 

P3. "edges of a central cut." You have not defined a central cut; you only defined a central set. 

P3. "into normed space" => "into normed spaces" 

P4. The same notation $f$ has been used for multiple purposes: flow-cut gap constant on page 3, a face of the planar graph on page 3, and now the embedding. 

P4. "maximum congestion". The notion of congestion should be defined here. 

P6. How is G_f defined for the infinite face? 

P6. spacing in ",i.e." 

P6. The notation G\C and G[C] are in conflict with standard notation; I was confused by this notation, for example, in Claim 1, where I thought G\C is the graph obtained by removing vertices in C. I think you should redefine this notation. 

P6. S^1_f$ is defined for a non-infinite face only. If so, it's good to mention this somewhere around this paragraph. Otherwise, I don't see why R(S^i_f) subset R(S^{i+1}_f), in particular, S^1_f will be some cycle inside G, and then by definition R(S^i_f) does not contain f. 

P6. I found the notation $S_f$ somewhat confusing; maybe $S_f^{\infty}$ is a better alternative as it is easier to remember that you are taking the limit to infinity. 

P7. The notation P(.,.) used in the proof of Lemma 2 is somewhat confusing: for P(u1,v1) and P(u2,v2) they are shortest paths, while for x1,y1, P(x1,y1) might not be. Maybe using Q for the path from x1 to y1? 

P7. Proof of Lemma 2 is sloppy, I think. You seem to assume that P(u2,v2) intersects with P(u1,v1) in a very specific way: the subpath from x2 to y2 of P(u1,v1) contains both x1 and y1. But I don't see why this is the only case. I can think of two other cases: 

Case 1, P(x1,y1) and P(u2,v2) do not intersect. For this case, I imagine the path P(u1,v1) wraps around f2 so that f2 is inside the finite region enclosed by P(u1,v1) and a path between u1 and v1 along f. Then, in this case, P(u2,v2) might not intersect P(u1,v1) at all. Also, P(x1,y1) is not unique as there are two paths along S^1_f. 

Case 2. P(u2,v2) does not wrap around f1; in other words, it only intersects, for example, the subpath from v1 to y1 of P(x1,y1). In this case, the path after the replacement is not completely inside S^1_{f2}. 


P8. The last sentence o the proof of Lemma 3, " hence R = R(S1_{f1})=R(S1_{f2})". should be \not= instead of =. 

P8. Proof of Lemma 4. I think you would need to choose P to be a minimal shortest path satisfying the assumption. Otherwise, you could have a portion of P going out of the region, and hence the claim that R(T_f) \subset R(S_f^1) is not true. 

P9. $u,v\in S_{g_i}$, what is $S_{g_i}$? 

P9. "There exists $u,v \in f_I$," and the proof of Claim 2 seems to suggest that the definition of alpha-loose on P8, is that for every u,v in S_f instead of for every u,v in f. So I am confused here. 

P9. "Hence if u,v in G_i, then d_{G_i}(u,v) = d_{G}(u,v)". I am confused about the "if u,v in G_i" part. Both vertices are the endpoints of P and by definition, belong to both G_i, no? 

P10. "Then the statement of the theorem holds for non-geodesic face f1". I interpret this sentence as saying that you would consider f1 as the (new) infinite face and apply the theorem to f1. (If I am correct, I suggest making this explicit in writing.) The definition alpha-loose applies to S_f, but now it is not clear why it holds true for the S_{f_I}. The assumption is only for f_I. 

P11. I found the notation $S_f^i$ here confusing, as $S_f$ was already used for the support of f. 

P11. "vertices in C(f)," do you mean V(f)? The same C(f) appears elsewhere. 

P11. $g= 1/7 (h + h_0 + ...)$ should point out that the + operation means coordinate concatenation. 

P14. $\delta_{R}(u,w) = 3$, $R$ should be caligraphic. 

P14. "i.e." => "i.e.," 

P14. $l$ is used both as the maximum index of f and the length function. 

P15. It's helpful to remind readers at this point what is a central cut. 

P15. Theorem 12, you should define the notion of an alpha-loose cycle from the start. The definition currently only applies to a support of a face. 

P15. "a alpha-loose" => "an alpha-loose" 

P15. "it immediately follows that for any uv in S, d_H1(uv)\geq d_G(uv)". I think the author should include proof for this fact; as far as I can see, the proof is not immediate. 

P15. "geodesic pairs in G_2" => "geodesic pairs in G_1" 

P16. the last 3 equations at the end of the page, to get from the 1st equation to the 2nd one, the author should add a note somewhere that d_H1(u,u_1) = d_G(u,u_1)/\alpha and the same for v,v1. 


P17. By "\alpha-loose face," do you mean a face where its support is alpha-loose? If so, then you should note that. The definition of alpha-loose, as it is written, only applies to the support of a face, not to a face itself. 


P17. I was confused with the notation G1 here. G1 in Lemma 12 denotes the inner part of the cycle, but here the outer part of the cycle. 

P17. The author should explain why the induction does not reduce the length exponentially over the course of the induction. To be more explicit, first, the algorithm reduces the length by alpha and then recurses on G1. There is a potential that the length will be reduced further by alpha in the recursion on G1 and so on. 

P17. Overall I found the proof of Theorem 13 to be too concise, making it hard to follow. Claims like "by induction hypothesis and statement of Theorem 12" pack many things in a very short sentence. 

The reference section should be better formatted; several ell1 notations in the titles are inconsistent.

